Model reduction of dynamical systems on nonlinear manifolds using deep convolutional autoencoders

Nearly all model-reduction techniques project the governing equations onto a linear subspace of the original state space. Such subspaces are typically computed using methods such as balanced truncation, rational interpolation, the reduced-basis method, and (balanced) POD. Unfortunately, restricting the state to evolve in a linear subspace imposes a fundamental limitation to the accuracy of the resulting reduced-order model (ROM). In particular, linear-subspace ROMs can be expected to produce low-dimensional models with high accuracy only if the problem admits a fast decaying Kolmogorov $n$-width (e.g., diffusion-dominated problems). Unfortunately, many problems of interest exhibit a slowly decaying Kolmogorov $n$-width (e.g., advection-dominated problems). To address this, we propose a novel framework for projecting dynamical systems onto nonlinear manifolds using minimum-residual formulations at the time-continuous and time-discrete levels; the former leads to manifold Galerkin projection, while the latter leads to manifold least-squares Petrov--Galerkin (LSPG) projection. We perform analyses that provide insight into the relationship between these proposed approaches and classical linear-subspace reduced-order models; we also derive a posteriori discrete-time error bounds for the proposed approaches. In addition, we propose a computationally practical approach for computing the nonlinear manifold, which is based on convolutional autoencoders from deep learning. Finally, we demonstrate the ability of the method to significantly outperform even the optimal linear-subspace ROM on benchmark advection-dominated problems, thereby demonstrating the method's ability to overcome the intrinsic $n$-width limitations of linear subspaces.

==> writeup_arXiv_revision(round1)_local_copy/analysis.tex <==
\section{Analysis}\label{sec:analysis}
We now perform analysis of the proposed \GalerkinName\ and \LSPGName\
projection methods. For notational simplicity, this section omits the
dependence of operators on parameters $\param$.
\begin{proposition}[Affine trial manifold recovers classical Galerkin and
	LSPG]\label{thm:affine}
	If the trial manifold is affine,
	then \LSPGName\ projection is equivalent to classical linear-subspace LSPG projection. 
	If additionally the decoder mapping associates with an orthgonal matrix,
	then \GalerkinName\ projection is equivalent to classical linear-subspace Galerkin
	projection.
	\begin{proof}
	If the trial manifold is affine, then the decoder
		can be expressed as the linear mapping
		\begin{equation} \label{eq:linearDecoder}
			\rdbasisnl:\drdstate\mapsto\rdbasis
		\drdstate 
\end{equation} 
		with $\rdbasis\in\RR{\nstate\times\nstatered}$.\\
		\noindent \underline{\GalerkinNameCap}.
		Substituting the linear decoder \eqref{eq:linearDecoder} into the
		\GalerkinName\ ODE \eqref{eq:cont_rom} yields
\begin{align} \label{eq:cont_romGalOne}
	\difftime{\rdstate}(t\paramSemiProof) =
	\rdbasis\pseudoinv
	\velo\left(\stateRef\paramParProof + \rdbasis\rdstate(t\paramSemiProof),
	t\paramSemiProof
	\right),\quad \rdstate(0\paramSemiProof)=\zero.
\end{align}
		Similarly, substituting the linear decoder \eqref{eq:linearDecoder}
		into
the \GalerkinName\ O$\Delta$E Eq.~\eqref{eq:GalerkinODeltaE} yields the same
		system, but with the residual defined as
		\begin{equation} \label{eq:galModResidual}
			\rdres^n:\grdstate\gparamSemiProof \mapsto\rdbasis\pseudoinv \res^{n}
			(\stateRef\gparamParProof +
	 \rdbasis \grdstate^n\gparamSemiProof).
	  \end{equation} 
		If additionally the trial-basis matrix is orthogonal, i.e.,
		then 
		$\rdbasis\pseudoinv = \rdbasis\tran$ and the ODE \eqref{eq:cont_romGalOne}
		is equivalent to the
		classical Galerkin ODE
\begin{align} \label{eq:cont_romGal}
	\difftime{\rdstate}(t\paramSemiProof) =
	\rdbasis\tran
	\velo\left(\stateRef\paramParProof + \rdbasis\rdstate(t\paramSemiProof),
	t\paramSemiProof
	\right),\quad \rdstate(0\paramSemiProof)=\zero,
\end{align}
		while the O$\Delta$E residual \eqref{eq:galModResidual} is equivalent to the
		classical Galerkin O$\Delta$E residual
 \begin{equation} 
	 \rdres^n:\grdstate\gparamSemiProof \mapsto\rdbasis\tran \res^{n}
	 (\stateRef\gparamParProof +
	 \rdbasis \grdstate^n\gparamSemiProof).
	  \end{equation} 
		\noindent \underline{\LSPGNameCap}.
Substituting the linear decoder \eqref{eq:linearDecoder} into the \LSPGName\
		O$\Delta$E \eqref{eq:lspg_proj} yields the classical LSPG O$\Delta$E
\begin{align}\label{eq:lspg_projLinear}
	\rdtestbasis^{n}(\rdstate^{n}\paramSemiProof)\tran
	\res^{n}\left(\stateRef\paramParProof +
	\rdbasis\rdstate^n\paramSemiProof\right) = \zero
\end{align}
with classical LSPG test basis 
\begin{align*}
\rdtestbasis^{n}:\grdstate\gparamSemiProof &\mapsto 
	\left( \alpha_0
	\identity - \Delta t \beta_0 \frac{\partial \velo}{\partial \dstate}
	\left( \stateRef\gparamParProof + \rdbasis\grdstate, t^n\gparamParProof \right) \right)
	\rdbasis.
\end{align*}

	\end{proof}
\end{proposition}


The \GalerkinName\ O$\Delta$E
\eqref{eq:GalerkinODeltaE}--\eqref{eq:time_cont_res} was derived using a
project-then-discretize approach, as we formulated the residual-minimization
problem \eqref{eq:cont_opt_problem} at the time-continuous level, and
subsequently discretized the equivalent ODE \eqref{eq:cont_rom} in time. We
now derive conditions under which an equivalent model could have been derived
using a discretize-then-project approach, i.e., by substituting the
approximated state $\states \leftarrow \aprxstate$ defined in
Eq.~\eqref{eq:state_approx} into the FOM O$\Delta$E \eqref{eq:fomODeltaE} and
subsequently premultiplying the overdetermined system by a test basis.

\begin{theorem}[Commutativity of time discretization and \GalerkinName\
	projection]\label{prop:comm}
For \GalerkinName\ projection, time discretization and projection are commutative if 
	either (1) the 
	trial manifold corresponds to an affine subspace, or (2) 
	the nonlinear trial manifold is
	twice continuously differentiable;
	$\|\rdstate^{n-j} - \rdstate^{n}\| = \bigO(\Delta t)$ for all
	$n\innatno{\ntime}$, $j\innatno{k}$; and
	the limit
	$\Delta t\rightarrow 0$ is taken.
	%If additionally the reduced-basis matrix
	%associated with the decoder is orthogonal, then both methods recover
	%classical Galerkin projection.
	%In both cases, the test basis applied to the time-discrete corresponds to the transpose of the
	%pseudoinverse of the Jacobian of the decoder, i.e., 
	%$\testBasisGal = [\jacrdbasisnl(\rdstate)\pseudoinv]^T$.
\end{theorem}
\begin{proof}
	 The discrete residual
characterizing	
	the \GalerkinName\ O$\Delta$E \eqref{eq:GalerkinODeltaE}, which
	was derived using a project-then-discretize approach,
	 is defined as $\rdres^n$ in Eq.~\eqref{eq:time_cont_res}.\\
%\begin{equation} \label{eq:manifoldGalODeltaE}
%\sum_{j=0}^{k} \alpha_j \rdstate^{n-j} - \Delta t \sum_{j=0}^{k} \beta_j
%\jacrdbasisnl(\rdstate^{n-j})\pseudoinv \velo(
%\stateRef+\rdbasisnl(\rdstate^{n-j}),t^{n-j}\gparamSemiProof)=\zero.
%\end{equation} 
\noindent Substituting the approximated state $\states \leftarrow \aprxstate$ defined in
	Eq.~\eqref{eq:state_approx} into the FOM O$\Delta$E \eqref{eq:fomODeltaE}
	yields
$\res^{n}(\stateRef+\rdbasisnl(\rdstate^n)\paramSemiProof) =
	\zero$.
%or equivalently
%\begin{align}\label{eq:fomODeltaEGalTwo}
%\sum_{j=0}^{k} \alpha_j \rdbasisnl(\rdstate^{n-j})
	%- \Delta t \sum_{j=0}^{k} \beta_j \velo (
	%\stateRef+\rdbasisnl(\rdstate^{n-j}), t^{n-j}\paramSemiProof)=\zero,
%\end{align}
	%where we have used $\sum_{j=0}^k\alpha_j=0$. Eq.~\eqref{eq:fomODeltaEGalTwo}
	This is an overdetermined system of equations and thus may not have a
	solution. As such, we perform projection by enforcing orthgonality of this
	residual to a test basis $\testBasisGal:\RR{\nstatered}\rightarrow\RR{\nstate\times\nstatered}$ such
	that the discretize-then-project \GalerkinName\ O$\Delta$E corresponds to 
	$\rdresDisc^n(\rdstate^n)=\zero$ with 
 \begin{equation} 
	 \rdresDisc^n:\grdstate\mapsto\testBasisGal(\grdstate)^T\res^{n}(\stateRef+\rdbasisnl(\grdstate)\paramSemiProof).
	  \end{equation} 
	The discretize-then-project \GalerkinName\ ROM is equivalent to the proposed
	\GalerkinName\ ROM if and only if there exists a full-rank matrix
	$\constantSymbGal:\RR{\nstatered}\timesparamspaceProof\rightarrow\RRstar{\nstatered\times\nstatered}$
	such that
	\begin{equation}\label{eq:matchingGal}
\rdres^n(\grdstate\gparamSemiProof)=\constantAnalysisGal\rdresDisc^n(\grdstate\gparamSemiProof).
	\end{equation}
	\noindent \textit{Case 1.} 	We now consider the general (non-asymptotic)
	case.  
	Eq.~\eqref{eq:matchingGal} holds for any sequence of approximate
	solutions $\rdstate^n$, $n=1,\ldots,\ntime$ if and only if
	each term in this expansion matches, i.e.,
		\begin{align}\label{eq:requirementOneGal}
		\begin{split}
			\grdstate=&
			\constantAnalysisGal\testBasisTransposeAnalysisGal\rdbasisnl(\grdstate)\\
 \jacrdbasisnl(\grdstate)\pseudoinv \velo(
			\stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)=&
			\constantAnalysisGal\testBasisTransposeAnalysisGal\velo(
	 \stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)\\
			\rdstate^{n-j}=&\constantAnalysisGal\testBasisTransposeAnalysisGal\rdbasisnl(\rdstate^{n-j})\\
\jacrdbasisnl(\rdstate^{n-j})\pseudoinv \velo(
			\stateRef+\rdbasisnl(\rdstate^{n-j}),t^{n-j}\gparamSemiProof)=&
			\constantAnalysisGal\testBasisTransposeAnalysisGal \velo (
	 \stateRef+\rdbasisnl(\rdstate^{n-j}), t^{n-j}\gparamSemiProof),
			\end{split}
		\end{align}
where we have used $\sum_{j=0}^k\alpha_j=0$.
	We first consider the first and third conditions of
	\eqref{eq:requirementOneGal}.
	Because the inverse of a nonlinear operator---if it
		exists---must also be nonlinear, a necessary condition for these two
		requirements is that the trial manifold corresponds is affine
		such that the decoder satisfies \eqref{eq:linearDecoder}.
		Substituting Eq.~\eqref{eq:linearDecoder} into the first and third of
		the conditions of \eqref{eq:requirementOneGal} yields
		\begin{align}\label{eq:requirementTwoGal}
		\begin{split}
			\grdstate=&
			\constantAnalysisGal\testBasisTransposeAnalysisGal\rdbasis \grdstate \\
			\rdstate^{n-j}=&\constantAnalysisGal\testBasisTransposeAnalysisGal\rdbasis \rdstate^{n-j}
			\end{split}
		\end{align}
		for $j=1,\ldots,k$. A necessary and sufficient conditions for these to
		hold is
\begin{equation} \label{eq:constantDefGal}
	\constantAnalysisGal= \constantDefAnalysisGal.
\end{equation} 
We now consider the second and fourth conditions of
\eqref{eq:requirementOneGal}.
Substituting Eqs.~\eqref{eq:linearDecoder} and \eqref{eq:constantDefGal} into
these conditions yields
		\begin{align}\label{eq:requirementOneLinearGal}
		\begin{split}
 \rdbasis\pseudoinv \velo(\stateRef\gparamParProof +
			\rdbasis\grdstate,t^n\gparamSemiProof)=&
			\constantDefAnalysisGal\testBasisTransposeAnalysisGal\velo(\stateRef\gparamParProof +
	 \rdbasis\grdstate,t^n\gparamSemiProof)\\
\rdbasis\pseudoinv \velo(\stateRef\gparamParProof +
			\rdbasis\rdstate^{n-j},t^{n-j}\gparamSemiProof)=&
			\constantDefAnalysisGal\testBasisTransposeAnalysisGal \velo (\stateRef\gparamParProof +
	 \rdbasis\rdstate^{n-j}, t^{n-j}\gparamSemiProof)
			\end{split}
		\end{align}
		for $j=1,\ldots,k$. Noting that $\rdbasis\pseudoinv =
		[\rdbasis\tran\rdbasis]^{-1}\rdbasis\tran$, a necessary and sufficient
		condition for \eqref{eq:requirementOneLinearGal} to hold is 
		$
\rdbasis\pseudoinv = 
\constantDefAnalysisGal\testBasisTransposeAnalysisGal.
$
Because $\rdbasis$ has no dependence on the generalized state, the test basis
must also be independent of the generalized state, which yields
\begin{equation}\label{eq:finalEquivCondition}
	\rdbasis\pseudoinv =
	[\testBasisAnalysisGalNo^T\rdbasis]^{-1}\testBasisAnalysisGalNo^T.
\end{equation}
%\begin{equation} \label{eq:finalEquivCondition}
	%\rdbasis = \testBasisAnalysisGal.
%\end{equation} 
Thus, without using any asymptotic arguments, the proposed \GalerkinName\ ROM
could have been derived using a discretize-then-project approach if and only
if the test basis $\testBasisAnalysisGalNo$ applied to the overdetermined FOM
O$\Delta$E acting on the trial manifold satisfies
Eq.~\eqref{eq:finalEquivCondition}.
Examples of test bases that satisfy this condition include
$\testBasisAnalysisGalNo = [\rdbasis\pseudoinv]\tran$ and
$\testBasisAnalysisGalNo = \scalarConstant\rdbasis$ for some nonzero scalar
$\scalarConstant\in\RR{}$.
\\
\textit{Case 2.} We now consider asymptotic arguments.
	Assuming the nonlinear trial manifold is
	twice continuously differentiable, and
	$\|\rdstate^{n-j} - \rdstate^{n}\| = \bigO(\Delta t)$, then for $\grdstate$
	in a neighborhood of $\rdstate^n$ such that 
	$\|\grdstate - \rdstate^{n}\| = \bigO(\Delta t)$, we have
\begin{align} \label{eq:limiting}
	\begin{split}
		\jacrdbasisnl(\rdstate^{n-j})\pseudoinv &=
		\jacrdbasisnl(\rdstate^{n})\pseudoinv + \bigO(\Delta t)\\
	\jacrdbasisnl(\grdstate)\pseudoinv &=
		\jacrdbasisnl(\rdstate^{n})\pseudoinv + \bigO(\Delta t)\\
	\rdbasisnl(\rdstate^{n-j}) &= \rdbasisnl(\rdstate^{n}) + \jacrdbasisnl(\rdstate^{n})[
\rdstate^{n-j}-\rdstate^{n}
	]
	+ \bigO(\Delta t)\\
	\rdbasisnl(\grdstate) &= \rdbasisnl(\rdstate^{n}) + \jacrdbasisnl(\rdstate^{n})[
\grdstate-\rdstate^{n}
	]
	+ \bigO(\Delta t).
	\end{split}
\end{align} 
Substituting these expressions into the definition of the
discretize-then-project \GalerkinName\ residual $\rdresDisc^n$ and enforcing
equivalence of each term in  the matching conditions
\eqref{eq:matchingGal} and taking the limit $\Delta t\rightarrow 0$ yields
		\begin{align}\label{eq:requirementOneGalAsymp}
		\begin{split}
			\grdstate=&
			\constantAnalysisGal\testBasisTransposeAnalysisGal
			\jacrdbasisnl(\rdstate^{n})
			\grdstate\\
 \jacrdbasisnl(\rdstate^n)\pseudoinv \velo(
			\stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)=&
			\constantAnalysisGal\testBasisTransposeAnalysisGal\velo(
	 \stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)\\
			\rdstate^{n-j}=&\constantAnalysisGal\testBasisTransposeAnalysisGal
			\jacrdbasisnl(\rdstate^{n})
			\rdstate^{n-j}\\
\jacrdbasisnl(\rdstate^{n})\pseudoinv \velo(
			\stateRef+\rdbasisnl(\rdstate^{n-j}),t^{n-j}\gparamSemiProof)=&
			\constantAnalysisGal\testBasisTransposeAnalysisGal \velo (
	 \stateRef+\rdbasisnl(\rdstate^{n-j}), t^{n-j}\gparamSemiProof),
			\end{split}
		\end{align}
		where we have used $\sum_{j=0}^k\alpha_j=0$.
A necessary and sufficient condition for the first and
third conditions to hold is
\begin{equation} 
\constantAnalysisGal = 
	[\testBasisTransposeAnalysisGal
			\jacrdbasisnl(\rdstate^{n})]^{-1}.
	\end{equation} 
	Then, a necessary and sufficient condition for the second and fourth
	conditions to hold is
	 \begin{equation} \label{eq:finalEquivConditionAsy}
\jacrdbasisnl(\rdstate^n)\pseudoinv = 
[\testBasisTransposeAnalysisGal
			\jacrdbasisnl(\rdstate^{n})]^{-1}
\testBasisTransposeAnalysisGal.
		  \end{equation} 
Examples of test bases that satisfy Eq.~\eqref{eq:finalEquivConditionAsy}
include 
$\testBasisAnalysisGal = [\jacrdbasisnl(\rdstate^{n})\pseudoinv]\tran$ and 
$\testBasisAnalysisGalNo = \scalarConstant\jacrdbasisnl(\rdstate^{n})$ for
some nonzero scalar
		$\scalarConstant\in\RR{}$.
%If additionally the reduced basis matrix is orthogonal such that
%$\rdbasis\tran\rdbasis=\identity$, then $\rdbasis\pseudoinv=\rdbasis\tran$
%and so both O$\Delta$Es recover the classical Galerkin O$\Delta$E
%\begin{align}\label{eq:fomODeltaEGalFive}
%\sum_{j=0}^{k} \alpha_j \rdbasis\tran\rdstate^{n-j}
%- \Delta t \sum_{j=0}^{k} \beta_j \rdbasis\tran\velo (\initstate(\param) +
%\rdbasis\rdstate^{n-j}, t^{n-j}; \param)=\zero.
%\end{align}
\end{proof}
Theorem \ref{prop:comm} shows that \GalerkinName\ can be derived using a
discretize-then-project approach for nonlinear trial manifolds. This shows
that previous analysis \cite[Theorem 3.4]{carlbergGalDiscOpt} related to
commutativity of (residual-minimizing) Galerkin projection and time
discretization extends to the case of nonlinear trial manifolds.

We now show that the limiting equivalence result reported in \cite[Section
5]{carlbergGalDiscOpt} between Galerkin and LSPG projection for linear
subspaces also extends to nonlinear trial manifolds.

\begin{theorem}[Limiting equivalence]\label{thm:equivalence}
	\GalerkinNameCap\ and \LSPGName\ are equivalent if 
	either (1) the trial
	manifold corresponds to an affine subspace
	and either an explicit scheme is
	employed or the limit $\Delta t\rightarrow 0$ is taken, or (2) the
	nonlinear manifold is twice continuously differentiable; $\|\rdstate^{n-j} -
	\rdstate^{n}\| = \bigO(\Delta t)$ for all $n\innatno{\ntime}$,
	$j\innatno{k}$; and the limit $\Delta t\rightarrow 0$ is taken.
\end{theorem}
\begin{proof}
	The proof follows similar steps to those applied in the proof of Theorem
	\ref{prop:comm}.
	The discrete residual $\rdresLSPGn$ defined in \eqref{eq:lspg_projsimple},
	which characterizes the \LSPGName\ O$\Delta$E \eqref{eq:lspg_proj}, can be
	written as
	\begin{align} \label{eq:LSPGODeltaEResFull}
 \begin{split} 
	 \rdresLSPGn:\grdstate\gparamSemiProof\mapsto&
	\alpha_0\rdtestbasis^{n}(\grdstate\gparamSemiProof)\tran\rdbasisnl(\grdstate) - \Delta t \beta_0
	\rdtestbasis^{n}(\grdstate\gparamSemiProof)\tran\velo(
	 \stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof) + \\
	 & \sum_{j=1}^{k} \alpha_j 
	 \rdtestbasis^{n}(\grdstate\gparamSemiProof)\tran\rdbasisnl(\rdstate^{n-j})
	 - \Delta t \sum_{j=1}^{k}\beta_j \rdtestbasis^{n}(\grdstate\gparamSemiProof)\tran \velo (
	 \stateRef+\rdbasisnl(\rdstate^{n-j}), t^{n-j}\gparamSemiProof)
 \end{split} 
	  \end{align} 
%\begin{align*} 
%\begin{split} 
%\rdresLSPGn:(\grdstate;\gparam)\mapsto&
%\jacrdbasisnl (\grdstate)\tran\left( \alpha_0
%\identity - \Delta t \beta_0 \frac{\partial \velo}{\partial \dstate}
%\left(\initstate(\gparam)  + \rdbasisnl(\grdstate), t^n;\gparam \right)
%\right)\tran\times\\
%&\left(
%\alpha_0\rdbasisnl(\grdstate) - \Delta t \beta_0
%\velo(\initstate(\gparam) +
%\rdbasisnl(\grdstate),t^n;\gparam) + \sum_{j=1}^{k} \alpha_j 
%\rdbasisnl(\rdstate^{n-j})
%- \Delta t \sum_{j=1}^{k} \beta_j \velo (\initstate(\gparam) +
%\rdbasisnl(\rdstate^{n-j}), t^{n-j};
%\gparam)\right),
%\end{split} 
%\end{align*} 
		where we have used $\sum_{i=0}^k\alpha_i=0$. \LSPGNameCap\ projection is
		equivalent to \GalerkinName\ projection if and only if the O$\Delta$Es
		characterizing the two methods are equivalent, which is equivalent
		to requiring the existence of a full-rank matrix
		$\constantSymb:\RR{\nstatered}\timesparamspaceProof\rightarrow\RRstar{\nstatered\times\nstatered}$ such that
		\begin{equation}\label{eq:conditionsMatchL}
		\rdresn(\grdstate\gparamSemiProof)=\constantAnalysis\rdresLSPGn(\grdstate\gparamSemiProof).
		\end{equation}
			
		\noindent\textit{Case 1.} We now consider the general (non-asymptotic)
		case. Eq.~\eqref{eq:conditionsMatchL} holds for any sequence of
		approximate solutions 
		$\rdstate^n$, $n=1,\ldots,\ntime$
if and only if each term in this expansion matches, i.e.,
		\begin{align}\label{eq:requirementOne}
		\begin{split}
			\grdstate=&
			\constantAnalysis\testBasisTransposeAnalysis\rdbasisnl(\grdstate)\\
 \jacrdbasisnl(\grdstate)\pseudoinv \velo(
			\stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)=& \constantAnalysis\testBasisTransposeAnalysis\velo(
	 \stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)\\
			\rdstate^{n-j}=&\constantAnalysis\testBasisTransposeAnalysis\rdbasisnl(\rdstate^{n-j})\\
\jacrdbasisnl(\rdstate^{n-j})\pseudoinv \velo(
			\stateRef+\rdbasisnl(\rdstate^{n-j}),t^{n-j}\gparamSemiProof)=&
			\constantAnalysis\testBasisTransposeAnalysis \velo (
	 \stateRef+\rdbasisnl(\rdstate^{n-j}), t^{n-j}\gparamSemiProof)
			\end{split}
		\end{align}
		for $j=1,\ldots,k$.
		Comparing Conditions \eqref{eq:requirementOne} with
		\eqref{eq:requirementOneGal}, we see that the requirements are the same as
		in Theorem \ref{prop:comm}, but with 
		$\testBasis$ replacing $\testBasisGal$ and  $\constantSymb$ replacing
		$\constantSymbGal$. Thus, we arrive at the same result: necessary and
		sufficient conditions for equivalence are that
the trial manifold corresponds to an affine
		subspace such that the decoder satisfies \eqref{eq:linearDecoder}
		and  the test basis $\testBasisAnalysis$ satisfies
\begin{equation} \label{eq:lspgGenCond}
\rdbasis\pseudoinv = \constantDefAnalysis\testBasisTransposeAnalysis.
\end{equation} 
Note that necessary conditions for Eq.~\eqref{eq:lspgGenCond} to hold are
$\range(\testBasisAnalysis) = \range(\rdbasis)$.
Examples of test basis that satisfy this condition include
$\testBasisAnalysis = [\rdbasis\pseudoinv]\tran$ and 
$\testBasisAnalysis = \scalarConstant\rdbasis$ for some nonzero scalar
		$\scalarConstant\in\RR{}$.
However, unlike in Theorem \ref{prop:comm}, we are not free to choose the
test basis; rather, it is defined as 
 \begin{equation} \label{eq:lspgTestOverall}
\rdtestbasis^{n}:\grdstate\mapsto\testBasisAnalysisLongLinear.
	  \end{equation}
		For the necessary condition
$\range(\testBasisAnalysis) = \range(\rdbasis)$ to hold, the second term in 
Eq.~\eqref{eq:lspgTestOverall} must be zero. This occurs if and only if either
(1) an explicit scheme is
	employed such that $\beta_0=0$, or (2) the limit $\Delta t\rightarrow 0$ is
	taken. In both cases, 
	$
	\testBasisAnalysis=\scalarConstant\rdbasis$
	holds with
		$\scalarConstant=\alpha_0$.\\
		\noindent
\noindent\textit{Case 2.} We now consider asymptotic arguments.
Assuming the nonlinear trial manifold is
	twice continuously differentiable, and
	$\|\rdstate^{n-j} - \rdstate^{n}\| = \bigO(\Delta t)$, then for $\grdstate$
	in a neighborhood of $\rdstate^n$ such that 
	$\|\grdstate - \rdstate^{n}\| = \bigO(\Delta t)$, we obtain the expressions
	\eqref{eq:limiting}.
Substituting these expressions into the definition of the $\rdresLSPGn$ in
Eq.~\eqref{eq:LSPGODeltaEResFull},
enforcing
equivalence of each term in  the matching conditions
\eqref{eq:conditionsMatchL}, and taking the limit $\Delta t\rightarrow 0$ yields
		\begin{align}\label{eq:requirementOneAsymp}
		\begin{split}
			\grdstate=&
			\constantAnalysis\testBasisTransposeAnalysis
			\jacrdbasisnl(\rdstate^{n})
			\grdstate\\
 \jacrdbasisnl(\rdstate^n)\pseudoinv \velo(
			\stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)=&
			\constantAnalysis\testBasisTransposeAnalysis\velo(
	 \stateRef+\rdbasisnl(\grdstate),t^n\gparamSemiProof)\\
			\rdstate^{n-j}=&\constantAnalysis\testBasisTransposeAnalysis
			\jacrdbasisnl(\rdstate^{n})
			\rdstate^{n-j}\\
\jacrdbasisnl(\rdstate^{n})\pseudoinv \velo(
			\stateRef+\rdbasisnl(\rdstate^{n-j}),t^{n-j}\gparamSemiProof)=&
			\constantAnalysis\testBasisTransposeAnalysis \velo (
	 \stateRef+\rdbasisnl(\rdstate^{n-j}), t^{n-j}\gparamSemiProof),
			\end{split}
		\end{align}
		where we have used $\sum_{j=0}^k\alpha_j=0$.  
	A necessary and sufficient condition for the first and
	third conditions to hold is 	
 \begin{equation} 
\constantAnalysis = 
	 [\testBasisTransposeAnalysis\jacrdbasisnl(\rdstate^{n})]^{-1}.
	  \end{equation} 
		Then, 
	a necessary and sufficient condition for the second and fourth
	conditions to hold is
	 \begin{equation} \label{eq:finalEquivConditionAsyL}
\jacrdbasisnl(\rdstate^n)\pseudoinv = 
[\testBasisTransposeAnalysis
			\jacrdbasisnl(\rdstate^{n})]^{-1}
\testBasisTransposeAnalysis.
		  \end{equation} 
		As in Case 1 above, a necessary condition for \eqref{eq:finalEquivConditionAsyL}
		to hold is that $\range(\testBasisAnalysis) =
		\range(\jacrdbasisnl(\rdstate^n))$. Due to the definition of the test
		basis, this requires the second term on the right-hand side of Eq.~\eqref{eq:testBasisMatDef}
		to be zero. This is already satisfied by the stated assumption that the
		limit $\Delta t\rightarrow 0$ is taken, in which case $
		\testBasisAnalysis=\scalarConstant\jacrdbasisnl (\grdstate)$ holds with
		$\scalarConstant=\alpha_0$. It can be easily verified that this test basis
		satisfies the condition \eqref{eq:finalEquivConditionAsyL}.
\end{proof}
%\begin{proposition}[Discrete-time error bounds]
	%\KTC{TODO}
%\end{proposition}


==> writeup_arXiv_revision(round1)_local_copy/drawbacks.tex <==
We note that one drawback of the method in its current form (relative to
classical linear-subspace methods) is that it incurs a costlier training
process, as training a deep convolutional autoencoder is significantly more
computationally expensive than simply computing the left singular vectors of a
snapshot matrix. In addition, the proposed method is characterized by
significantly more hyperparameters---which relate to the autoencoder
architecture---than classical methods.


==> writeup_arXiv_revision(round1)_local_copy/error_analysis.tex <==
We now derive \textit{a posteriori} local discrete-time error bounds for both
the manifold Galerkin and manifold LSPG projection methods in the context of
linear multistep methods, and demonstrate that manifold LSPG projection
sequentially minimizes the error bound in time. For notational simplicity, we
suppress the second argument of the velocity $\velo$, as the time superscript
appearing in the second argument always matches that of the first argument.
%These results
%follow closely the steps employed in \cite[Section
%5]{carlbergGalDiscOpt} between Galerkin and LSPG projection for linear
%subspaces also extends to nonlinear trial manifolds.

\begin{theorem}[Error bound]\label{thm:error_bound}
	If the velocity $\velo$ is Lipschitz continuous, i.e.,
	there exists a constant $\lipschitz>0$ such that
	$\norm{\velo(\bm{x})-\velo(\bm{y})}\leq\lipschitz\norm{\bm{x}-\bm{y}}$
	for all $\bm{x},\,\bm{y}\in\RR{\nstate}$, and
	the time step is sufficiently small such that
	$ \Delta t < {\abs{\alpha_0}}/{\abs{\beta_0}\lipschitz}$,
	then 
\begin{align} 
	\label{eq:boundGal}&\norm{\stateFOMArg{n} \negstateROMGalArg{n}}\leq\frac{1}{\hconstant}
	\norm{\resnROMArg{\stateROMGalArg{n}}} +
\sum_{j=1}^{k}\gammaconstantj\norm{
\stateFOMArg{n-j}\negstateROMGalArg{n-j}
		}\\
	\label{eq:boundLSPG}&\norm{\stateFOMArg{n} \negstateROMLSPGArg{n}}\leq\frac{1}{\hconstant}
	\min_{\dstate\in\stateRef+ \manifold}\norm{\resnROMArg{\dstate}} +
\sum_{j=1}^{k}\gammaconstantj\norm{
\stateFOMArg{n-j}\negstateROMLSPGArg{n-j}
		},
\end{align} 
	where $\rdstateGal^n$ denotes the manifold Galerkin solution satisfying 
	\eqref{eq:GalerkinODeltaE} and $\rdstateLSPG^n$
	denotes the manifold LSPG solution satisfying \eqref{eq:disc_opt_problem}.
	Here, $\hconstant\defeq\abs{\alpha_0} - \abs{\beta_0}\lipschitz\Delta t$
and $\gammaconstantj\defeq\left(\abs{\alpha_j} + 
	\abs{\beta_j}\lipschitz
	\Delta
	t\right)/\hconstant$.
\end{theorem}
\begin{proof}
	We begin by defining linear multistep residual operators associated with the
	FOM sequence of solutions $\{\stateFOMArg{j}\}_{j=1}^n$ and an (arbitrary)
	sequence of approximate solutions $\{\stateROMArg{j}\}_{j=1}^n$, i.e.,
	\begin{align}
		\resnFOM:\dstate&\mapsto\alpha_0 \dstate - \Delta t \beta_0
		\velo(\dstate) + \sum_{j=1}^{k} \alpha_j \stateFOMArg{n-j}
	- \Delta t \sum_{j=1}^{k} \beta_j \velo (\stateFOMArg{n-j})\\
		\resnROM:\dstate&\mapsto
		\alpha_0 \dstate - \Delta t \beta_0
		\velo(\dstate) + \sum_{j=1}^{k} \alpha_j \stateROMArg{n-j}
	- \Delta t \sum_{j=1}^{k} \beta_j \velo (\stateROMArg{n-j}).
	\end{align}
We note that $\stateROMArg{j} = \stateROMGalArg{j}$, $j=1,\ldots,n$ in the case of manifold
Galerkin projection, and 
$\stateROMArg{j} = \stateROMLSPGArg{j}$, $j=1,\ldots,n$ in the case of manifold
LSPG projection.
Subtracting  $\resnROMArg{\stateROMArg{n}}$ from $\resnFOMArg{\stateFOMArg{n}}$ and
noting from 
Eq.~\eqref{eq:fomODeltaE} that $\resnFOMArg{\stateFOMArg{n}} =
\zero$ yields
\begin{align*} 
\begin{split} 
	-\resnROMArg{\stateROMArg{n}} &= \alpha_0\left(\stateFOMArg{n} -
	\stateROMArg{n}\right) - \Delta
	t\beta_0\left(\velo(\stateFOMArg{n})-\velo(\stateROMArg{n})\right)
	 + \sum_{j=1}^{k} \alpha_j
	 \left(\stateFOMArg{n-j}-\stateROMArg{n-j}\right)
	- \Delta t \sum_{j=1}^{k} \beta_j \left(\velo (\stateFOMArg{n-j})
	-\velo (\stateROMArg{n-j})\right).
\end{split} 
\end{align*} 
Rearranging this expression gives
\begin{align} \label{eq:IandII}
\begin{split} 
	&\underbrace{\stateFOMArg{n} - \stateROMArg{n} - 
	\frac{\Delta
	t\beta_0}{\alpha_0}\left(\velo(\stateFOMArg{n})-\velo(\stateROMArg{n})\right)}_\text{(I)}
	 =\\
	&\qquad\underbrace{-\frac{1}{\alpha_0}\resnROMArg{\stateROMArg{n}} -  \frac{1}{\alpha_0}\sum_{j=1}^{k} \alpha_j
	 \left(\stateFOMArg{n-j}-\stateROMArg{n-j}\right)
	+ \frac{\Delta t}{\alpha_0} \sum_{j=1}^{k} \beta_j \left(\velo (\stateFOMArg{n-j})
	-\velo (\stateROMArg{n-j})\right)}_\text{(II)}.
\end{split} 
\end{align} 
We proceed by bounding $\norm{\text{(I)}}$ from below, and $\norm{\text{(II)}}$ from above.
To bound $\norm{\text{(I)}}$ from below, we apply the reverse triangle to obtain
 \begin{equation} \label{eq:Iboundone}
	 \norm{\text{(I)}}\geq
	 \abs{
	 \norm{\stateFOMArg{n} - \stateROMArg{n}} - 
	 \norm{\underbrace{
\frac{\Delta
	 t\beta_0}{\alpha_0}\left(\velo(\stateFOMArg{n})-\velo(\stateROMArg{n})\right)
		 }_\text{(I.a)}}
	 }.
 \end{equation}
 We now use Lipschitz continuity of the velocity $\velo$ to bound
 $\norm{\text{(I.a)}}$ from above as
\begin{equation} \label{eq:Iboundtwo}
\norm{
	\text{(I.a)}
}\leq \frac{\Delta t
		 \abs{\beta_0}\lipschitz}{\abs{\alpha_0}}\norm{\stateFOMArg{n} -
		 \stateROMArg{n}}.
\end{equation} 
If time-step-restriction condition $ \Delta t < {\abs{\alpha_0}}/{\abs{\beta_0}\lipschitz}$ holds,
then we can combine inequalities \eqref{eq:Iboundone} and \eqref{eq:Iboundtwo}
as
\begin{equation} \label{eq:Ilowerbound}
\norm{\text{(I)}}\geq
	 \frac{\hconstant}{\abs{\alpha_0}}\norm{\stateFOMArg{n} - \stateROMArg{n}}.
\end{equation} 

To bound $\norm{\text{(II)}}$ in Eq.~\eqref{eq:IandII} from above, we apply the triangle
inequality and employ Lipschitz continuity of the velocity $\velo$, which
gives
\begin{equation} \label{eq:IIupperbound}
	\norm{
		\text{(II)}
		}\leq
	\frac{1}{\abs{\alpha_0}}\norm{\resnROMArg{\stateROMArg{n}}}
	+ \frac{1}{\abs{\alpha_0}}\sum_{j=1}^{k}\left(\abs{\alpha_j} + 
	\abs{\beta_j}\lipschitz
	\Delta
	t\right)\norm{
\stateFOMArg{n-j}-\stateROMArg{n-j}
		}.
\end{equation} 
Combining Eq.~\eqref{eq:IandII} with inequalities \eqref{eq:Ilowerbound} and
\eqref{eq:IIupperbound} gives
\begin{equation} \label{eq:finalGenResult}
	\norm{\stateFOMArg{n} - \stateROMArg{n}}\leq\frac{1}{\hconstant}
	\norm{\resnROMArg{\stateROMArg{n}}} +
\sum_{j=1}^{k}\gammaconstantj\norm{
\stateFOMArg{n-j}-\stateROMArg{n-j}
		}.
\end{equation} 
The manifold-Galerkin error bound \eqref{eq:boundGal} results from substituting
$\stateROMArg{j} = \stateROMGalArg{j}$, $j=1,\ldots,n$ in \eqref{eq:finalGenResult}, while
the manifold-LSPG error bound \eqref{eq:boundLSPG} results from substituting
$\stateROMArg{j} = \stateROMLSPGArg{j}$, $j=1,\ldots,n$ in \eqref{eq:finalGenResult}
and noting that the manifold LSPG solution $\stateROMLSPGArg{j}$ satisifies the
time-discrete residual-minimization property \eqref{eq:disc_opt_problem}.
\end{proof}

This result illustrates that the time-discrete residual minimization property
of manifold LSPG projection allows its approximation to sequentially minimize
the error bound, as the first term on the right-hand side of bound \eqref{eq:boundLSPG}
corresponds to the new contribution to the error bound at time instance $t^n$,
while the second term on the right-hand side comprises the recursive term in
the bound.

